Nematicity and superconductivity: Competition versus cooperation

Electronic nematic behavior has been identified and studied in iron-based superconductors for some time, particularly in the well-known BaFe$_2$As$_2$ system, where it is well-known to compete with superconductivity. On the other hand, it has been shown recently that FeSe displays a negligible effect of nematicity on superconductivity near the superconducting transition, and actual cooperation between the two orders when the system is doped with S. Recently it has also been proposed that LiFeAs undergoes a nematic transition in the superconducting state itself. Generally, we expect superconductivity to be anisotropic when it coexists with nematic order, but it is not clear under what circumstances the two orders compete or cooperate, nor how the anisotropy of the superconducting state correlates with that in the nematic state. To address this, we study a simple mean field model of a $d$-wave Pomeranchuk instability together with a mixed $s,d$ pairing interaction, and identify when nematicity is enhanced or suppressed by superconductivity. We show that the competition or cooperation depends significantly on the distortion of the Fermi surface due to nematicity relative to the anisotropy of the superconducting gap function. Further, we discuss the implications of our results for FeSe and LiFeAs.

==> qmdefs.tex <==
% Derivatives
\def\dx{{\partial \over \partial x}}
\def\dy{{\partial\over\partial y}}
\def\dz{{\partial\over\partial z}}
\def\dxx{{\partial^2\over\partial x^2}}
\def\dyy{{\partial^2\over\partial y^2}}
\def\dzz{{\partial^2\over\partial z^2}}
\def\Dx#1{{\partial #1\over \partial x}}
\def\Dy#1{{\partial #1\over \partial y}}
\def\Dz#1{{\partial #1\over \partial z}}
\def\Dzz#1{{\partial^2 #1\over \partial z^2}}
\def\Dyy#1{{\partial^2 #1\over \partial y^2}}
\def\Dxx#1{{\partial^2 #1\over \partial x^2}}
\def\Dt#1{{\partial #1 \over \partial t}}
\def\dphi{{\partial\over\partial \phi}}
\def\dth{{\partial\over\partial \theta}}
\def\dr{{\partial\over \partial r}}
\def\Dphi#1{{\partial #1\over \partial \phi}}
\def\Dth#1{{\partial #1\over \partial \theta}}
\def\Dr#1{{\partial #1\over \partial r}}
\def\Drr#1{{\partial^2 #1\over\partial r^2}}
\def\dt{{\partial\over \partial t}}
\def\dert{{d\over dt}}
\def\dtau{{\partial\over \partial \tau}}
\def\Dtau#1{{\partial #1\over \partial\tau}}
\def\Dert#1{{d #1\over d t}}
\def\Derx#1{{d #1\over d x}}
\def\Derrr#1{{d^2 #1\over d r^2}}
\def\Derr#1{{d #1\over dr}}
\def\derx{{d\over dx}}
% Bolds
\def\k{{\bf k}}
\def\r{{\bf r}}
\def\R{{\bf R}}
\def\q{{\bf q}}
\def\p{{\bf p}}
\def\x{{\bf x}}
\def\yvec{{\bf y}}
\def\xvec{{\bf x}}
\def\rvec{{\bf r}}
\def\qvec{{\bf q}}
\def\kvec{{\bf k}}
\def\pvec{{\bf p}}
\def\pvh{{\hat{\bf p}}}
\def\jvec{{\bf j}}
\def\Avec{{\bf A}}
\def\Bvec{{\bf B}}
\def\Evec{{\bf E}}
\def\Fvec{{\bf F}}
\def\Lvec{{\bf L}}
\def\Jvec{{\bf J}}
\def\Pvec{{\bf P}}
\def\Rvec{{\bf R}}
\def\Svec{{\bf S}}
\def\dvec{{\bf d}}
\def\vvec{{\bf v}}
% Hats
\def\ih{{\hat i}}
\def\jh{\hat j}
\def\kh{\hat k}
\def\hatn{\hat n}
\def\hath{{\hat h}}
\def\hatA{{\hat A}}
\def\hatB{{\hat B}}
\def\hatC{{\hat C}}
\def\hatD{{\hat D}}
\def\hatF{{\hat F}}
\def\hatH{{\hat H}}
\def\hatJ{{\hat J}}
\def\hatK{{\hat K}}
\def\hatL{{\hat L}}
\def\hatS{{\hat S}}
\def\hatV{{\hat V}}
\def\hatQ{\hat Q}
\def\hatp{\hat p}
\def\hatP{\hat P}
\def\hatO{\hat O}
\def\O{\hat{\cal O}}
\def\hatr{{\hat r}}
\def\hatT{{\hat T}}
\def\hatU{\hat U}
\def\hatN{\hat N}
\def\rvh{{\hat{\bf r}}}
\def\hatpsi{{\hat\psi}}
\def\hatrho{{\hat\rho}}
\def\hatpsidag{{\hat\psi}^\dagger}
% Bras and kets
\def\psiket{|\psi\rangle}
\def\psibra{\langle\psi |}
\def\phiket{|\phi\rangle}
\def\phibra{\langle\phi |}
\def\xket{|x\rangle}
\def\xbra{\langle x |}
\def\pket{|{\bf p}\rangle}
\def\pbra{\langle {\bf p} |}
\def\rket{|{\bf r}\rangle}
\def\nket{| n\rangle}
\def\nbra{\langle n |}
\def\mket{| m\rangle}
\def\mbra{\langle m |}
\def\rbra{\langle {\bf r} |}
\def\ket#1{|#1\rangle}
\def\bra#1{\langle #1|}
\def\vacket{\ket{0}}
\def\vacbra{\bra{0}}
\def\vac{\vacket}
\def\dket{\ket{\downarrow}}
\def\uket{\ket{\uparrow}}
\def\dbra{\bra{\downarrow}}
\def\ubra{\bra{\uparrow}}
% Math symbols
\def\paulix{\left[\begin{array}{cc}0 & 1\\1 & 0\end{array}\right]}
\def\pauliy{\left[\begin{array}{cc}0&-i\\i&0\end{array}\right]}
\def\pauliz{\left[\begin{array}{cc}1&0\\0&-1\end{array}\right]}
\def\up{\uparrow}
\def\down{\downarrow}
\def\bigint{\displaystyle\int}
\def\Tr{{\rm Tr}}
\def\ve{\varepsilon}
\def\dg#1{#1^\dagger}
\def\adag{a^\dagger}
\def\bdag{b^\dagger}
\def\cdag{c^\dagger}
\def\Adag{A^\dagger}
\def\Bdag{B^\dagger}
\def\Cdag{C^\dagger}
\def\psidag{\psi^\dagger}
% Spacing & layout
\def\sp{\vskip .2cm\noindent}
\def\bsp{\sp\sp}
% Bold operators (hats)
\def\Sop{{\bf{\hat S}}}
\def\Lop{\bf{\hat L}}
\def\Jop{\bf{\hat J}}
% Misc.
\def\T{{\cal T}}
\def\Lz{\hat{L}_z}
\def\Lsq{\hat{L}^2}
\def\pre{-{\hbar^2\over 2m}}
\def\psic{\psi^*}
\def\avg#1{\langle #1 \rangle}
\def\={&=&}
\def\mybox#1{\fbox{\mbox{$\displaystyle #1 $}}}
\def\aks{a_{\k\sigma}}
\def\adks{\adag_{\k\sigma}}
